Approximating the Quadratic Transportation Metric in Near-Linear Time

Computing the quadratic transportation metric (also called the $2$-Wasserstein distance or root mean square distance) between two point clouds, or, more generally, two discrete distributions, is a fundamental problem in machine learning, statistics, computer graphics, and theoretical computer science. A long line of work has culminated in a sophisticated geometric algorithm due to Agarwal and Sharathkumar in 2014, which runs in time $\tilde{O}(n^{3/2})$, where $n$ is the number of points. However, obtaining faster algorithms has proven difficult since the $2$-Wasserstein distance is known to have poor sketching and embedding properties, which limits the effectiveness of geometric approaches. In this paper, we give an extremely simple deterministic algorithm with $\tilde{O}(n)$ runtime by using a completely different approach based on entropic regularization, approximate Sinkhorn scaling, and low-rank approximations of Gaussian kernel matrices. We give explicit dependence of our algorithm on the dimension and precision of the approximation.

==> sections/main_old.tex <==
% !TEX root = ../stoc.tex
\section{Approximating $W_2$ in $\tilde{O}(n)$ time}\label{sec:alg}

\begin{algorithm}[H]
\begin{algorithmic}[1]
\Require{$X := \{x_1, \dots, x_n\} \subset \RR^{d}$, $\p \in \Delta_n$, $\q \in \Delta_n$, $\eps > 0$}
\Ensure{$\hat P \in \Coup$, $\hat W \in \RR$}
\State $\eps \gets \min(\eps,5)$, $\eta \gets \tfrac{20 \log n}{\eps}$, $M \gets \tfrac{300 \log n}{\eps}$
\State $\tilde K \gets V_M(x_1,\dots,x_n;\tfrac{1}{\sqrt{2\eta}})^TV_M(x_1,\dots,x_n;\tfrac{1}{\sqrt{2\eta}})$ \label{line:taylor} \Comment Compute low-rank approximation
\State $(D_1, D_2) \gets \textsc{Sinkhorn}(\tilde K, \p, \q, \tfrac{\eps}{10})$ \label{line:sinkhorn} \Comment Approximate Sinkhorn projection
\State $\Phat \gets \textsc{Round}(D_1 \tilde K D_2, \p, \q)$, in the form $\Phat = D_1'\tilde K D_2' + vw^T$ \Comment Round to feasible set
\label{line:round}
\State $\hat W \gets \sum_{i,j=1}^n P_{ij} \|x_i - x_j\|^2$ \Comment Compute objective value
\label{line:obj}
\State \Return{$\Phat$,  $\hat W$}
\end{algorithmic}
\caption{\ALG \todo rename}
\label{alg:main}
\end{algorithm}

Pseudocode for our proposed algorithm is given in Algorithm~\ref{alg:main}. It returns a feasible matrix $\hat P \in \Coup$ as well as its objective value $\hat W$. We emphasize that the matrix $\hat P$ is returned in factored form (of rank $\leq m+1$), since otherwise even writing this $n \times n$ matrix down would require $\Omega(n^2)$ time. This factored form may enable scalable implementations of algorithms that use $\hat P$ later in the computational pipeline. For instance, we show how to leverage this low-rank factored form to show that steps~\ref{line:taylor},~\ref{line:sinkhorn},~\ref{line:round}, and~\ref{line:obj} are all implementable in $o(n^2)$ time. Implementation details are deferred to Subsection~\ref{subsec:main:proof}. Finally, we note that all steps in Algorithm~\ref{alg:main} are easily parallelizable since everything can be written as matrix-vector products.
\par The following theorem -- the main result of the paper -- shows that $\hat W$ is within $\eps$ additive error of the true $2$-Wasserstein distance between $p$ and $q$.

\begin{theorem}\label{thm:main}
There is an implementation of Algorithm~\ref{alg:main} such that for any $\{x_1, \dots, x_n\} \subset \ball$, any $p,q \in \Delta_n$, and any $\eps > 0$, the algorithm terminates in \todo time and returns a feasible matrix $\Phat \in \Coup$ (in factored form) and scalar $\hat W = \sum_{i,j=1}^n P_{ij} \|x_i - x_j\|^2$ such that $\hat W \leq W_2^2(\p, \q) + \eps$.
%\footnote{The notation $\tilde O$ hides factors of the form $(\log n)^\alpha(\log(1/\delta))^\beta(\log(1/\ep))^\gamma$ for constants $\alpha, \beta, \gamma$. We employ the subscripts to stress that the constant depends on the quantities $d, \eta, R$.}
\end{theorem}

By taking a suare root of $\hat{W}$, this gives an answer to Problem~\ref{prob:coup}.

\begin{cor}\label{cor:main}
\ja{Write for $W_2(p,q)$ without square.}
\end{cor}


For the rest of this section, $x_1, \dots, x_n \in \ball$ are fixed, $C \in \RR^{n \times n}$ denotes the cost matrix with entries $C_{ij} := \|x_i - x_j\|^2$, and $K \in \RR^{n \times n}$ denotes the entrywise exponentiated matrix $K_{ij} := \exp(- \eta C_{ij})$.

\note{FB: here I would put some paragraph explaining how we are going to proceed, that is,  technical lemmas then theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Helpful lemmas}\label{subsec:main:approx-cost}

First, we establish that $\tilde{K}$ is a sufficiently good approximation to $K$ for our purposes.

\begin{lemma}\label{lem:logK-to-K}
Let $\tilde{K}$ be as in Algorithm~\ref{alg:main}. Then each entry $\tilde{K}_{ij} \geq \half e^{-\eta}$, and moreover the matrix $\tilde{C} \in \RR^{n \times n}$ with entries $\tilde{C}_{ij} := \eta^{-1} \log \tilde{K}_{ij}$ satisfies $\|C - \tilde{C}\|_{\infty} \leq \frac{\eps}{10}$.
%\[
%\|\log K - \log \tilde{K} \|_{\infty} \leq 1.
%\]
\end{lemma}
\begin{proof}
By Lemma~\ref{lem:taylor-gaussian}, Stirling's inequality, and our choice of $M = \tfrac{300 \log n}{\eps} \geq 2e^2 \eta$, we have $
\|K - \tilde{K}\|_{\infty}
\leq \tfrac{(2\eta)^M}{M!}
\leq  \tfrac{1}{\sqrt{2\pi M}} (\frac{2\eta e}{M})^M
\leq \half e^{-2e^2\eta}
\leq \half e^{-\eta}$.
Thus since the smallest element of $K$ has size at least $e^{-\eta}$, the reverse triangle inequality gives that $\Ktilde_{ij} \geq K_{ij} - |K_{ij} - \Ktilde_{ij}| \geq \half e^{-\eta}$. Next, this inequality implies that $|\log K_{ij} - \log \tilde K_{ij}|
\leq \frac{|K_{ij} - \tilde K_{ij}|}{\min(K_{ij}, \tilde{K}_{ij})}
\leq \frac{\half e^{-\eta} }{\half e^{-\eta}}
= 1$, from which we conclude that $\|C - \tilde{C}\|_{\infty} = \eta^{-1} \|\log K - \log\tilde{K}\|_{\infty} \leq \eta^{-1} = \tfrac{\eps}{20 \log n} \leq \tfrac{\eps}{10}$.
\end{proof}


%Next, we establish that the variational problem defining Wasserstein distance is stable with respect to perturbing the marginals of the transport polytope (the feasible set) in total-variation distance. Note that this result is independent of the cost metric.


%\begin{lemma}\label{lem:feas-stability}
%Consider any $\p,\p',\q,\q' \in \Delta_n$ and $\Ctilde \in \RR^{n \times n}$. Let $P^* \in \min_{P \in \Coup} \langle P, \Ctilde \rangle$ and let $Q^* \in \min_{P' \in \Coupp} \langle P', \Ctilde \rangle$ be any minimizers. Then
%\[
%\abs{\langle P^*, \Ctilde \rangle - \langle Q^*, \Ctilde \rangle}
%\leq \|\Ctilde\|_{\infty} \Bigg(\|\p - \p'\|_1 + \|\q - \q'\|_1\Bigg).
%\]
%\end{lemma}
%\begin{proof}
%By Lemma~\ref{lem:round-alg}, there exists a matrix $G \in \Coupp$ such that $\|G - P^*\|_1 \leq \|\p - \p'\|_1 + \|\q - \q'\|_1$. Thus
%$\langle Q^*, \Ctilde \rangle
%\leq
%\langle G, \Ctilde \rangle 
%=
%\langle G-P^*, \Ctilde \rangle + \langle P^*, \Ctilde \rangle
%\leq \|\Ctilde\|_{\infty} (\|\p - \p'\|_1 + \|\q - \q'\|_1) + \langle P^*, \Ctilde \rangle$. The other direction follows by symmetry.
%\end{proof}


%\begin{lemma}\label{lem:feas-stability}
%For any $\p,\p',\q,\q' \in \Delta_n$ and any $\Ctilde \in \RR^{n \times n}$,
%\[
%\abs{\left( \min_{P \in \Coup} \langle P, \Ctilde \rangle \right) - \left( \min_{P' \in \Coupp} \langle P', \Ctilde \rangle \right)}
%\leq \|\Ctilde\|_{\infty} \Bigg(\|\p - \p'\|_1 + \|\q - \q'\|_1\Bigg).
%\]
%\end{lemma}
%\begin{proof}
%Fix any minimizer $P^* \in \argmin_{P \in \Coup} \langle P, \Ctilde \rangle$. By Lemma~\ref{lem:round-alg}, there exists a matrix $G \in \Coupp$ such that $\|G - P^*\|_1 \leq \|\p - \p'\|_1 + \|\q - \q'\|_1$. Thus
%$\min_{P' \in \Coupp} \langle P', \Ctilde \rangle
%\leq
%\langle G, \Ctilde \rangle 
%=
%\langle G-P^*, \Ctilde \rangle + \langle P^*, \Ctilde \rangle
%\leq \|\Ctilde\|_{\infty} (\|\p - \p'\|_1 + \|\q - \q'\|_1) + \min_{P \in \Coup} \langle P, \Ctilde \rangle$. The other direction follows by symmetry.
%\end{proof}







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of the main theorem (Theorem~\ref{thm:main})}\label{subsec:main:proof}

\paragraph*{Approximation guarantee.}
\par Let $\tilde{C} \in \RR^{n \times n}$ be the matrix with entries $\tilde{C}_{ij} := - \eta^{-1} \log \tilde{K}_{ij}$; this is well-defined since $\tilde{K}$ has strictly positive entries by Lemma~\ref{lem:logK-to-K}. Let $P^* \in \argmin_{P \in \Coup} \langle P, C \rangle$ be any optimal solution for the original problem, $P^{\eta} := \argmin_{P \in \Coup} \langle P, C \rangle - \eta^{-1} H(P)$ be the (unique) optimal solution to the regularized problem, and $\tilde{P} := \argmin_{P \in \Coup} \langle P, \tilde{C} \rangle - \eta^{-1} H(P)$ be the (unique) optimal solution to the regularized problem with the cost matrix $\tilde{C}$.
%$\tilde{P} = \Sinkcoup(e^{-\eta \tilde{C}})$
We bound the suboptimality gap $\langle \hat{P}, C \rangle - \langle P^*, C \rangle$ by decomposing it as:
\begin{align*}
\underbrace{\langle P^{\eta} - P^*, C \rangle}_\textbf{(i)}
+
\underbrace{\langle \tilde{P}, \tilde{C} \rangle - \langle \Peta, C \rangle}_\textbf{(ii)}
+
\underbrace{\langle D_1\tilde{K}D_2 - \tilde{P}, \tilde{C} \rangle}_\textbf{(iii)}
+
\underbrace{\langle \hat{P} - D_1\tilde{K}D_2 , \tilde{C} \rangle}_\textbf{(iv)}
+
\underbrace{\langle \hat{P}, C - \tilde{C} \rangle}_\textbf{(v)}
\end{align*}
It suffices to show that each of these terms is bounded above by $\tfrac{\eps}{5}$.
\begin{enumerate}
\item[(i)] By definition of $P^{\eta}$, $\langle  P^{\eta}, C \rangle - \eta^{-1}H(P^{\eta}) \leq \langle P^*, C \rangle - \eta^{-1}H(P^*)$. Since the entropy of a joint distribution on $[n] \times [n]$ is bounded within $[0,\log(n^2)]$~\citep[Theorem 2.6.4]{coverthomas}, we conclude that $\langle P^{\eta} - P^*, C \rangle \leq \eta^{-1}(H(P^{\eta}) - H(P^*)) \leq 2 \eta^{-1}\log n = \tfrac{\eps}{10}$.
\item[(ii)] By definition of $\tilde{P}$, $\langle \tilde{P}, \tilde{C} \rangle - \eta^{-1}H(\tilde{P}) \leq \langle P^{\eta}, \tilde{C} \rangle - \eta^{-1}H(P^{\eta})$. Thus $\langle \tilde{P}, \tilde{C} \rangle - \langle \Peta, C \rangle  \leq \eta^{-1} (H(\tilde{P}) - H(P^{\eta})) + \langle  P^{\eta}, \tilde{C} - C \rangle \leq 2\eta^{-1} \log n + \|\tilde{C} - C\|_{\infty} \leq \tfrac{\eps}{5}$ where we have used the same entropy bound as above, H\"older's inequality, and Lemma~\ref{lem:logK-to-K}.
%\item[(ii)] By Proposition~\ref{prop:kkt}, $P^{\eta} = \Sinkcoup(e^{-\eta C})$ and $\tilde{P} = \Sinkcoup(e^{-\eta \tilde{C}})$. Thus by applications of H\"older's inequality, Proposition~\ref{prop:sink-stable}, and then Lemma~\ref{lem:logK-to-K}, we conclude that
%$
%\langle C, \tilde{P} - P^{\eta} \rangle
%\leq \|C\|_{\infty} \|\tilde{P} - P^{\eta}\|_1
%\leq \|C\|_{\infty} \|\log K - \log \tilde{K}\|_{\infty}
%\leq \tfrac{\eps}{5}$.
%\item[(iii)] Again using H\"older's inequality and Lemma~\ref{lem:logK-to-K}, 
%$\langle \tilde{C} - C, \tilde{P}\rangle \leq \|\tilde{C} - C\|_{\infty} \|\tilde{P}\|_1 = \eta^{-1}\|\log K - \log \tilde{K}\|_{\infty} \leq \tfrac{\eps}{5}$.
\item[(iii)] Let $\p' := (D_1\tilde{K}D_2)\bone$ and let $\q' := (D_1\tilde{K}D_2)^T\bone$. Then by Proposition~\ref{prop:kkt}, $D_1\tilde{K}D_2 = \argmin_{P \in \Coup} \langle P, \tilde{C} \rangle - \eta^{-1}H(P)$. Thus by Lemma~\ref{lem:feas-stability}, 
\begin{align}
\abs{\langle D_1\tilde{K}D_2 - \tilde{P}, \tilde{C} \rangle} \leq \|\tilde{C}\|_{\infty} (\|\p - \p'\|_1 + \|\q - \q'\|_1).
\label{eq:proof-main:nasty}
\end{align}
This is bounded above by $\tfrac{\eps}{5}$ since $\|\p - \p'\|_1 + \|\q - \q'\|_1 \leq \tfrac{\eps}{10}$ by line~\ref{line:sinkhorn}, and since $\|\tilde{C}\|_{\infty} \leq \|C\|_{\infty} + \|C - \tilde{C}\|_{\infty} \leq 2$ by Lemma~\ref{lem:logK-to-K} and the fact that $\eps \leq 5$.
\item[(iv)] By H\"older's inequality and then Lemma~\ref{lem:round-alg}, $\langle \hat{P} - D_1\tilde{K}D_2, \tilde{C} \rangle \leq \|\tilde{C}\|_{\infty} \|\hat{P} - D_1\tilde{K}D_2\|_1 \leq  \|\tilde{C}\|_{\infty} (\|\p - \p'\|_1 + \|\q - \q'\|_1)$. This is bounded above by $\tfrac{\eps}{5}$ for the same reason as~\eqref{eq:proof-main:nasty}.
\item[(v)] By H\"older's inequality and Lemma~\ref{lem:logK-to-K}, $\langle \hat{P}, C - \tilde{C} \rangle \leq \|\hat{P}\|_1 \|C - \tilde{C}\|_{\infty} \leq \frac{\eps}{10}$.
\end{enumerate}


\paragraph*{Runtime guarantee.} All computations in Algorithm~\ref{alg:main} are done ``implicitly'' by only maintaining the matrices $\tilde{K}$, $D_1\tilde{K}D_2$, and $\hat{P}$ in factored form. Let $r := \binom{M-1+d}{d} \leq (\tfrac{(M+d)e}{d})^d = e^d \cdot \max(1,(\tfrac{M}{d})^d)$. Line~\ref{line:taylor} takes $O(nr)$ time by Lemma~\ref{lem:taylor-gaussian}, line~\ref{line:sinkhorn} takes $O(\frac{nr}{\eps}\log \tfrac{n}{\eps})$ time by Fact~\ref{fact:sink_run} and Lemma~\ref{lem:logK-to-K}, line~\ref{line:round} takes $O(nr)$ time by Lemma~\ref{lem:round-alg}, and line~\ref{line:obj} takes $O(ndr)$ time by Lemma~\ref{lem:quad-cost}.
%Finally, we show how line~\ref{line:obj} can be implemented quickly. A simple calculation gives $
%\sum_{i,j=1}^n P_{ij} \|x_i - x_j\|^2
%%= \sum_{i,j=1}^n P_{ij} \left(\|x_i\|^2 + \|x_j\|^2 - 2 x_i^T x_j \right)
%=
%- 2 \sum_{i,j=1}^n P_{ij} (X^TX)_{ij} 
%+ \sum_{i=1}^n (\p_i + \q_i )\|x_i\|^2$, where $X := [x_1 | \dots | x_n] \in \RR^{d \times n}$. The latter sum can clearly be computed in $O(nd)$ time. The former sum can be computed in $O(d(dn + nr + r^2))$ time using the simple and standard trace trick $\sum_{ij} P_{ij} (X^TX)_{ij} = \Tr(PX^TX) = \Tr(XPX^T) = \sum_{i=1}^{d} e_iXPX^Te_i$, where $e_i$ is the $i$th standard basis vector.
Finally, we note that throughout Algorithm~\ref{alg:main}, it suffices to use $O(\eta) = O(\eps^{-1} \log n)$ bits of precision since this suffices for the accuracy guarantee in Lemma~\ref{lem:logK-to-K}.
\qed

